Capturability-based Analysis of Legged Robot with Consideration of Swing Legs

Capturability of a robot determines whether it is able to capture a robot within a number of steps. Current capturability analysis is based on stance leg dynamics, without taking adequate consideration on swing leg. In this paper, we combine capturability-based analysis with swing leg dynamics. We first associate original definition of capturability with a time-margin, which encodes a time sequence that can capture the robot. This time-margin capturability requires consideration of swing leg, and we therefore introduce a swing leg kernel that acts as a bridge between step time and step length. We analyze N-step capturability with a combined model of swing leg kernels and a linear inverted pendulum model. By analyzing swing leg kernels with different parameters, we find that more powerful actuation and longer normalized step length result in greater capturability. We also answer the question whether more steps would give greater capturability. For a given disturbance, we find a step sequence that minimizes actuation. This step sequence is whether a step time sequence or a step length sequence, and this classification is based on boundary value problem analysis.

==> 3D_LIPM_Model_with_Finite_Foot.tex <==
\section{3D LIPM Model with Finite Foot}

In this section, we consider a LIPM model with finite foot. Its dynamic model is almost the same as the one without\cite{KarelRektorys2012}, except that $r_{ankle}$ are replaced with $r_{CoP}$, the equivalent center of pressure, in new functions. The equivalent center of pressure is a point that always lies within foot. We restate the dimensionless equations here.
\begin{equation}
r_{CoP} = r_{ankle} - \tau \times \hat{\mathbf{e}}_z
\label{eq:19}
\end{equation}
\begin{equation}
\ddot{r}_{CoM} = \mathbf{P}r_{CoM} - r_{CoP}
\label{eq:20}
\end{equation}
\begin{equation}
\dot{r}_{ic} = r_{ic} - r_{CoP}
\label{eq:21}
\end{equation}

We use a reference point in the following analysis. For simplicity, we pick it as the ankle location $r_{ref} = r_{ankle}$. In order to capture the robot, we wish $r_{CoP} \rightarrow r_{ic}$.
%With this limitation on earliest step time, we find it useful to make the following definition.
%\begin{definition}[$\Delta$-time invatiant $N$-step capurable]
%A state $X(t)$ is said to be \emph{$\Delta$-time invatiant $N$-step capurable}, 
%\end{definition}


==> README <==

September 17, 2014


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8a has a number of significant changes over the v1.8 release.
For a full list of changes, please read the file changelog.txt. The most
notable changes include:


 1) Extensive rework of the compsoc mode to comply with the latest standards
    of the IEEE Computer Society.

 2) Fixed abstract, index terms and diamond line for compsoc technotes.

 3) New \IEEEraisesectionheading{} command to provide for the special
    raised first section heading of Computer Society journal papers.

 4) Internal code improvements for page setup and command argument
    processing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> removed.tex <==

\begin{theorem}[1-step capturable for constrained LIPM at time $t$]
Given a LIPM with state $X(t)$ at time $t$, we add the following two limitations. 
\begin{enumerate}
	\item Its maximum foot step is $L \in \mathbb{R}^+$;
	\item It is able to step at time $t$.
\end{enumerate}
The state $X(t)$ is 1-step capturable if simultaneously the instant capture point $r_{ic}(t)$ lies within a circle centered at $r_{ankle}$ with a radius of $L$.
\label{thm:1-step capturable for LIPM-L}
\end{theorem}

With the help of Theorem~\ref{thm:1-step capturable for LIPM-L}, we have the following corollary.
\begin{corollary}
Suppose a constrained LIPM with maximum foot step $L$, and we assign it with a period $\delta$. Its state is $X(t)$ at time $t$. During the period, its state evolves from $X(t)$ to $X(t+\delta)$. 
The state $X(t+\delta)$ is 1-step capturable if at time $t+\delta$ the instant capture point $r_{ic}(t+\delta)$ lies within a circle centered at $r_{ankle}$ with a radius of $L$.
\end{corollary}

Combine Definition~\ref{def:margin 2-step} with Theorem~\ref{thm:1-step capturable for LIPM-L} and its corollary, we have the following theorem.
\begin{theorem}
Suppose robot is $\Delta_1$-margin $2$-step capturable at time $t_1$. %It has some $\Delta_1$-margin $2$-step capture points, denoting as $r_2$. 
A point $r_2 \in \mathbb{R}^2$ is a feasible\footnote{Here, feasible refers to within leg reach.}
 foot placement location at $t_1$. $r_2$ is a $\Delta_1$-margin $2$-step capture point, if the instant capture point $r_{ic}(t)$ lies within the circle centered at $r_2$ with radius $L$ for $t \in \left[t_1, t_1 + \Delta_1 \right]$, $i.e.$
\begin{equation}
\left| r_2 - r_{ic}(t)  \right| \leq L
\label{eq:judgement of delta 2-step}
\end{equation}
\label{thm:judgement of delta 2-step}
\end{theorem}

Using Equation~\ref{eq:ic evolve}, for time after $t_1$\footnote{We restate that $t_1$ is the time right after a step in made, so that $r_{ankle}$ in Equation~\ref{eq:ic evolve} is replaced with $r_2$, and $0$ with $t_1$.}, we have
\begin{equation}
\left| r_2 - r_{ic}(t)  \right| = \left| r_{ic}(t_{1}) - r_2 \right| \mathbf{e}^{\delta_1}
\label{eq:eq 2-10}
\end{equation}
where $\delta_1 \in \left[0, \Delta_1 \right]$. With Equations~\ref{eq:judgement of delta 2-step} and \ref{eq:eq 2-10}, a set of $\Delta_1$-margin $r_2$ at time $t_1$ can be found within the circle with radius 
\begin{equation}
R_2(t_1) = L \mathbf{e}^{-\Delta_1}
\label{eq:R_2}
\end{equation}
centered at $r_{ic}(t_1)$.
With larger $\Delta_1$, $R_2$ is smaller. This agrees with our intuition that if the required time margin $\Delta_1$ is greater, there should be less 2-step capture points with the time margin.

It is of great importance to understand physical meaning of the time margin $\Delta_1$. It ensures that the state after the step taking at time $t_1$ is 1-step capturable at least for $\Delta_1$ time. In real cases, $\Delta_1$ should be a value greater than $\Delta_e$, where $\Delta_e$ is the interval of the robot being able to step again after a step is finished. Only this satisfies could the robot make another step. The notion of $\Delta_1$-margin 2-step capture region gives a conservative estimate of 2-step capturability of state $X(t_1)$, requiring how the state should be after the stepping. Moreover, the greater $\Delta_1$ is, the more conservative the estimate is.


%It is of great importance to understand physical meaning of the time margin $\Delta_1$. $\Delta_1$ sets a upper bound of how slow a robot is allowed to step: it ensures that if a step is finished at time $t_1+\delta$, with $\delta \in \left[ 0, \Delta_1 \right]$, the state $X(t)$ being 1-step capturable for $t \in \left[t_1 + \delta, t_1 + \Delta_1 \right]$.\footnote{This also means that state $X(t_1 + \delta)$ before step is $\left(\Delta_1 - \delta \right)$-margin 2-step capturable.} In real cases, $\Delta_1$ should be a value greater than $\Delta_e$, where $\Delta_e$ is the interval of the robot being able to step again after a step is finished. The notion of $\Delta_1$-margin 2-step capture region gives a conservative estimate of 2-step capturability of state $X(t_1)$, and the greater $\Delta_1$ is, the more conservative the estimate is.

We now explore how this circle changes with respect to time after $t_1$. Suppose robot is $\Delta_1$-margin $2$-step capturable at time $t_1$, and it is able to step at $t_1$. However, it steps at a later time $t_1+\delta$, where $\delta > 0$, and its state $X(t_1+\delta)$ is also $\Delta_1$-margin $2$-step capturable. As the time margin requirement remains the same, the radius of the circle doesn't change, but its center moves from $r_{ic}(t_1)$ to $r_{ic}(t_1+\delta)$. The condition that state $X(t_1+\delta)$ is also $\Delta_1$-margin $2$-step capturable is satisfied, if the state $X(t_2)$, with $t_2 = t_1 - \Delta_2 > 0$, is $(\Delta_2 \Delta_1)$-margin 3-step capturable with $\Delta_2\geq \delta$ plus a foot placement at the corresponding $(\Delta_2 \Delta_1)$-margin 3-step capture point at $t_2$.

Hinted by this\footnote{In fact, it is a corollary of Definition~\ref{def:iterative N-step}.}, we have the following theorem that tells relation between time-margin $N$-step capturability with time-margin $(N-1)$-step capturability.
\begin{theorem}
Suppose a state $X(t_{N-1})$ is $\left( \Delta_{N-1} \cdots \Delta_1 \right)$-margin $N$-step capturable at time $t_{N-1}$. Then it is $( \Delta_{N-2}\cdots\Delta_1)$-margin $(N-1)$-step capturable at $t_{N-2}$ $\in$ $\left[t_{N-1}, t_{N-1}+\Delta_{N-1} \right]$, if a step is taken at the $\left( \Delta_{N-1} \cdots \Delta_1 \right)$-margin $N$-step capturable point at $t_{N-1}$. 
\label{thm:iterative t N-step}
\end{theorem}
If next step is done at $t_{N-2}^{step} \in \left[t_{N-1}, t_{N-1}+\Delta_{N-1} \right]$, such that the iteration continues. Iteratively applying Theorem~\ref{thm:iterative t N-step}, we have a conservative estimate of how long it will take for a state to be captured, as in the following theorem.
\begin{theorem}\footnote{Theorem~\ref{thm:iterative t N-step} and~\ref{thm:capture time} are general results. We discuss here for a better introduction of Question.}
Suppose a state $X(t_{N-1})$ is $\left( \Delta_{N-1} \cdots \Delta_1 \right)$-margin $N$-step capturable at time $t_{N-1}$. It can be captured with in $T_N= \sum_{i=1}^{N-1}{\Delta_i}$ from $t_{N-1}$.
\label{thm:capture time}
\end{theorem}
This estimate is conservative in a sense that there exists possibly smaller time $T$ within which the robot is still capturable. Theorem~\ref{thm:capture time} gives a sufficient but not necessary condition of time-margin $N$-step capturability. 
 
By now, it is natural to ask a question: 
given a state $X(t)$ with a sequence of $N-1$ time margins $\Delta_{N-1}, \cdots, \Delta_1$, is it possible to determine $X(t)$ is $(\Delta_{N-1} \cdots \Delta_1)$-margin $N$-step capturable or not?

We answer this question with the help of $(\Delta_{N-1} \cdots \Delta_1)$-margin $N$-step capture region. Recall in Theorem~\ref{thm:judgement of delta 2-step} and its discussion, we find the $\Delta_1$-margin 2-step capture region at time $t_1$ to be a circle with a time-invariant radius of $R_2$ and a center at $r_{ic}(t_1)$. If a step is not finished until a later time $t_1 + \delta$, this circle moves to a new center $r_{ic}(t_1+\delta)$. During this interval, the robot is $\Delta_1$-margin 2-step capturable if and only if the moving circle $C_2(t)$ and the leg length limit circle $C_{leg}(r_{ic}(t))$ is non-empty. Iteratively apply this, we have
\begin{equation}
\left| r_{ic}(t_{N} + \Delta_{N-1}) - r_N \right| \leq L+R_{N-1}
\label{eq:ite RN}
\end{equation}
where
\begin{equation}
r_{ic}(t_{N} + \Delta_{N-1}) = \left[r_{ic}(t_{N}) - r_{N}\right] \mathbf{e}^{\Delta_{N-1}} + r_N
\label{eq:ric at tN}
\end{equation}
So, the boundary of $r_N$ is the circle with a radius of 
\begin{equation}
R_N = (L+R_{N-1})\mathbf{e}^{-\Delta_{N-1}}
\label{eq:ite R_N}
\end{equation}
centered at its instant capture point $r_{ic}(t_N)$, $\forall N \geq 3$. We define $R_1 \equiv 0$, thus
\begin{equation}
R_N = (L+R_{N-1})\mathbf{e}^{-\Delta_{N-1}}
\label{eq:}
\end{equation} for $N\geq2$.
With this, we can have a group of isocentric circles that describes time-margin $N$-step capturablilty, which we define as follows.
\begin{definition}[time-margin capturability graph]
At time $t$, the instant capture point is at $r_{ic}$. We assign a sequence of time-margin denoted as $\Delta_{N-1}, \cdots, \Delta_1$, with $N \geq 2$. We have group of circles centered at instant capture point with radii defined by Equation~\ref{eq:R_2} and \ref{eq:ite R_N} for $N \geq 2$. The combined graph is called the \emph{time-margin $N$-step capturability graph}.
\label{def:graph}
\end{definition}
\begin{corollary}
The time-margin capturability graph is bounded.
\end{corollary}
\begin{IEEEproof}
We define $\Delta_m$ = $\min \Delta_i$, $\forall i \in [2, N]$.
From Equation~\ref{eq:ite R_N}, \begin{equation}
R_N \leq (L+R_{N-1}) \mathbf{e}^{-\Delta_m}
\label{eq:}
\end{equation}

Iteratively apply this, we have
\begin{equation}
R_N \leq L\mathbf{e}^{-\Delta_m} + \cdots + L \mathbf{e}^{-(N-2)\Delta_m} + R_2 \mathbf{e}^{-(N-2)\Delta_m}
\end{equation}
It converges, so the graph is bounded.
\end{IEEEproof}
The fact that the graph is bounded indicates that there are points $r \in \mathbb{R}^2$ that make states after stepping at $r$  not  capturable in sense of time-margin.

By now, we are able to give determinant of time-margin $N$-step capturablility. It is a broader version of Theorem~\ref{thm:1-step capturable for LIPM-L}. 
\begin{theorem}
Suppose the state of a LIPM-L at time $t$ is $X(t)$, and it is able to step. We assign a sequence of time margin denoted as $\Delta_{M-1}, \cdots, \Delta_1$. A time-margin capturablity graph $G$ can be found by Definition~\ref{def:graph}. We represent feasible foot step location of the LIPM-L at time $t$ as $A \subset \mathbb{R}^2$. If $G \cap A = \emptyset$, then then state is not $\Delta_{N-1}, \cdots, \Delta_1$-margin $N$-step capturable $\forall N \leq M$.
If a point $r \in G \cap A \neq \emptyset$, and it lies inside the circle with radius $R_N$, then it is $\Delta_{N-1}, \cdots, \Delta_1$-margin $N$-step capturable.
\label{thm:N-step CR}
\end{theorem}

As $R_N$ may be smaller than $R_{N-1}$, by Theorem~\ref{thm:N-step CR}, it is likely that a state is $\Delta_{N-1} \cdots \Delta_1$-margin $(N-1)$-step capturable while not $\Delta_{N} \cdots \Delta_1$-margin $N$-step capturable. This somehow contradicts with our intuition that the robot is more likely to succeed in becoming captured if it is required to take more steps. This contradiction comes from the intrinsic requirement expressed by $\Delta_{N-1}$. If we want $R_N > R_{N-1}$, the requirement that 
\begin{equation}
\Delta_{N-1} < ln\frac{L+R_{N-1}}{R_{N-1}}
\label{eq:}
\end{equation}
should be satisfied.
To simplify our analysis, we assume that $\Delta_i$ are equal to $\Delta_u$. This assumption makes sense, in that for a robot every step can be required to finish within a fixed time interval. With a uniform time margin, we have the following corollary.
\begin{corollary}
$R_N$ is increasing with respect to $N$ if $\Delta_i = \Delta_u$, $\forall i \in \mathbf{Z}^+$.
\label{clr:uniform R}
\end{corollary}
\begin{IEEEproof}
\begin{eqnarray}
R_N -R_{N-1} &=& \left(R_{N-1}-R_{N-2}\right) \mathbf{e}^{-\Delta_u} \nonumber \\
&=& \cdots \nonumber\\
&=& (R_2-R_1) \mathbf{e}^{-(N-2)\Delta_u} \nonumber \\
&=& L\mathbf{e}^{-(N-1)\Delta_u} > 0 
\label{eq:RN difference}
\end{eqnarray}
Thus, $R_N$ is increasing with respect to $N$.

We can also derive analytical expression for $R_N$ with fixed time-margin $\Delta_u$. With \eqref{eq:RN difference} and $R_1 = 0$, we find 
\begin{equation}
R_N = L \frac{\mathbf{e}^{-\Delta_u}-\mathbf{e}^{-N\Delta_u}}{1-\mathbf{e}^{-\Delta_u}}
\label{eq:R_N}
\end{equation}
where $N\in \mathbb{Z}^+$.
\end{IEEEproof}



With Theorem~\ref{thm:N-step CR} and Corollary~\ref{clr:uniform R}, we can design a bang-bang control algorithm regarding time-margin $N$-step capturability. Its input is state $X(t)$, and output is the set of points $r \in G \cap A$ that have the smallest value $N$. This controller ensures that the LIPM-L of state $X(t)$ is captured with least steps in the sense of $\Delta_u$-margin capturability. Geometrically speaking, the closer a step is made towards instant capture point, the better the step is in sense of $\Delta_u$ time margin capturability.

The bang-bang control assumes that the robot reach a largest distance within required time. This sometimes may not work. To resolve this, we design an optimization-based controller. We define the following definitions.















 \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figure/fs_nocons}
        \caption{unconstrained}
        \label{fig:nocons}
    \end{subfigure}
    %~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figure/ld1}
        \caption{$l_{max}/d = 1$}
        \label{fig:ld1}
    \end{subfigure}
   % ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figure/ld2}
        \caption{$l_{max}/d = 2$}
        \label{fig:ld2}
    \end{subfigure}
		\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figure/ld4}
        \caption{$l_{max}/d = 4$}
        \label{fig:ld4}
    \end{subfigure}
				\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figure/ld8}
        \caption{$l_{max}/d = 8$}
        \label{fig:ld8}
    \end{subfigure}
				\begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figure/ld16}
        \caption{$l_{max}/d = 16$}
        \label{fig:ld16}
    \end{subfigure}
    \caption{influence of $l_{max}/d$ on feasible set\\
		These figures illustrate how $l_{max}/k$ influences shape of feasible set, and consequently determines whether the solution is a step time or step length sequence. In these figures, $x$ axis is $\tau_1$, and $y$ axis is $\tau_2$. All figures shares same colorbar. Figure~\ref{fig:nocons} shows how an unconstrained feasible set should be. In other subfigures, regions that do not satisfy constraints are left blank. If $l_{max}/d$ is large (e.g. in \ref{fig:ld16}), global optimum is included, and this corresponds to a time sequence $\tau_{1,opt}$ and $\tau_{2,opt}$. If $l_{max}/d$ is small (e.g. in \ref{fig:ld2} to \ref{fig:ld8}), an optimum locates at the corner, which corresponds to $l_{max}$ at each step. If $l_{max}/d$ is too small, feasible set is empty, as in \ref{fig:ld1}. In this case, the state is not 2-step capturable.}
